Monocular Depth Estimation with Self-supervised Instance Adaptation

Recent advances in self-supervised learning havedemonstrated that it is possible to learn accurate monoculardepth reconstruction from raw video data, without using any 3Dground truth for supervision. However, in robotics applications,multiple views of a scene may or may not be available, depend-ing on the actions of the robot, switching between monocularand multi-view reconstruction. To address this mixed setting,we proposed a new approach that extends any off-the-shelfself-supervised monocular depth reconstruction system to usemore than one image at test time. Our method builds on astandard prior learned to perform monocular reconstruction,but uses self-supervision at test time to further improve thereconstruction accuracy when multiple images are available.When used to update the correct components of the model, thisapproach is highly-effective. On the standard KITTI bench-mark, our self-supervised method consistently outperformsall the previous methods with an average 25% reduction inabsolute error for the three common setups (monocular, stereoand monocular+stereo), and comes very close in accuracy whencompared to the fully-supervised state-of-the-art methods.

==> scratch.tex <==
\clearpage\newpage\section{Scratch}

When the ego-vehicle is stationary we must infer scene depth from a single view whereas when in motion we can utilise the multiple viewpoints available to determine depth \cite{scharstein2002a, Hartley2004}. Com

While monocular depth prediction is occasionally essential, in applications we are more often interested in working in a \emph{mixed setting}(where multiple views of a scene are available).
For example, in autonomous or assisted driving, a parked car, or a car stopped at a red light, does not move and thus requires us to perform single view depth prediction.
However, as soon as the car moves, multiple views become available and multi-view geometry can be used to further improve the reconstruction.
Working in a mixed setting can be done by combining monocular and multi-view reconstruction techniques; however, switching between different systems is complex, fragile and inefficient.

In this paper, we propose a new and very effective approach to work in a mixed monocular and multi-view reconstruction setting.
We note that self-supervised monocular depth estimation learns from certain relations of inputs rather than ground truth labels, namely the consistency between subsequent video frames~\cite{zhou2017} and stereo pairs\cite{monodepth17}.
We thus propose to take this one step further, by also exploiting self-consistency \textit{during inference} rather than just during training.
We show that, if we take an existing monocular depth prediction model and if we carefully select specific sub-components to optimize, we can update the relevant model parameters (weights) at inference time through standard back-propagation.
This step is optional, and is engaged only when motion is observed.

Doing so has two important benefits.
On the one hand, it leverages the strong monocular depth prediction prior to interpret motion data very robustly.
On the other hand, it uses self-supervised learning to further improve inference, learning continually.
We show this in two regimes:
(1) improving individual depth predictions and
(2) gradually improving the 3D prior over a longer sequence of input video frames.
The latter can also be interpreted as domain self-adaptation:
for instance, it also allows networks trained on datasets which may only be representative of driving in one location to be deployed in areas which may look different, automatically fine-tuning the model.
We also note that, whilst we experiment with monocular depth estimation, our idea of using self-supervision at inference time to improve predictions and to self-adapt a model is likely of far more general applicability.

The result is to consistently improve overall model accuracy when compared to the baseline monocular depth reconstruction model, as well other methods such as direct re-projection error minimization.

It follows that having a reliable and accurate monocular depth estimation method is critical, but one of the main challenges is not having enough labelled data to train these systems as monocular depth methods can only rely on prior information about real-world size and therefore distance of known objects, based on their visual appearance. In order to overcome the lack of labelled training data, which has to be generated using another sensing modality, self-supervised approaches have been recently applied to this problem\cite{monodepth17, monodepthv2, zhou2017, mancini2016fast}. In \textit{self-supervised learning}, certain relations or consistency of inputs rather than ground truth labels is exploited to train the system -- in depth estimation, the consistency between subsequent video frames or left/right images has been widely used\cite{monodepth17, zhou2017}.

In this paper, we propose to take self-supervised learning paradigm a step further, by also exploiting the principle of (self-)consistency \textit{during inference}. We show that if we take an existing model and if we carefully select specific sub-components to optimize, we can update the relevant model parameters (weights) at inference time through standard back-propagation to consistently improve overall model accuracy when compared to the base-line model.

Cameras allow us to recover a wide array of information about our surroundings from camera motion to instance segmentation. One weakness of monocular vision systems however is the depth ambiguity present in images. This becomes problematic as many desirable applications of vision systems: Augmented Reality, image editing and scene understanding. Currently circumvent this issue by using other sensors such as LiDAR, Radar or a stereo pair of images. These however induce other problems: LiDARs moving parts can break or become misaligned, can have problems in certain weather conditions\cite{Bijelic_2018}, produce sparse depth maps which may not be dense enough for some contexts and have a lower refresh rate when compared to many other sensors (10-15Hz\cite{velodyne64}). Radar performs better in adverse weather conditions but suffers with small objects, objects with low relative velocity and interference with other radar systems\cite{radar-shortcomings}. Stereo vision systems can also face problems with misalighment of cameras potentially spoiling outputs and lack of redundancy. Single image systems have some drawbacks as well, namely the collection of large training sets with ground truth data generated typically using another sensing modality.  Self-supervised approaches to depth estimation have recently shown promise with Monodepth\cite{monodepth17} showing that by warping images between a left and right stereo pair we can learn to predict depth maps for monocular images without ground truth information and SfMLearner\cite{zhou2017} showing how pose and depth networks can be trained with a sequence of images without a stereo pair.\\
We propose taking self-supervised training a step further and instead of freezing a networks weights to those learned on a test set we find that continually learning during inference time allows our network to develop a greater understanding of scenes local to our own system rather than the network only understanding those similar to it's test set. This allows networks trained on datasets which may only be representative of driving in one location to be deployed in areas which may look vastly different, allowing understanding of size for objects unseen in the training set.


In unsupervised Depth estimation we utilise ask our network learn novel view synthesis with the same viewpoint at another image in the sequence of frames. In doing this we aquire estimates of depth and pose as intermediate values  before the image warping is applied. This problem is however ill-posed owing to the ambiguity present in monocular image capture. We can address this by enforcing smoothness in depth maps and computing photo-consistency on patches when solving per-pixel depth by global optimization.\\
Our problem can therefore be phrased as minimisation of photometric error while training. With input frames $(I_t,I_{t'})$ where ($t$ is the current image and $t\prime$ an image temporally adjacent or from a stereo pair) our network produces a dense depth map $D_t = D(I_t)$ and then estimates pose $T_{t^\prime\to t'} = P(I_t,I_{t'})$ To train these networks we minimize photometric reprojection error $L_p$:

\begin{equation}
    L_p = \sum_{t'}pe(I_t,I_{t^\prime\to t})
    \label{eq:L_p}
\end{equation}
\begin{equation}
    I_{t^\prime\to t} = I_{t'} \Big\langle proj(D_t,T_{t^\prime\to t'},K)\Big\rangle
\end{equation}

Where $pe$ is photometric reconstruction error (L1 norm in pixel space) $proj()$ are the resulting 2D coordinates of projected depths $D_t$ and $I_t\prime$ and $\langle\rangle$ is the sampling operator. $K$ is the intrinsics of our camera (which can differ image to image if needs be). As in \cite{JaderbergSZK15} we use bilinear sampling to sample different sourse images in a locally sub-differentiably\cite{monodepthv2, lossfunctions} and use a combination of L1 and SSIM\cite{wang2004image}.\\
% In stereo training the relative pose of the other view is known whereas in monocular training pose can be predicted as in \cite{zhou2017} with another pose network which takes as input multiple frames for use in the reprojection.
Our loss also contains two contributions from Monodepthv2\cite{monodepthv2}: Per-pixel minimum reprojectino loss and stationary pixel automasking.\\
Instead of using the average reprojection error from our source frames ($I_{t\prime} \in \{I_{t-1},I_{t+1}\}$ for monocular and $I_{t\prime}$ is the opposite stereo view in stereo training) per-pixel minimum reprojection loss instead takes the minimum loss for a pixel along source images as otherwise our loss includes values where a patch has become occluded from one frame to the next resulting in high photometric error. With this consideration we modify equation \ref{eq:L_p} to be
% \begin{equation}
%     L_p = \min_{t\prime}pe(I_t,I_{t\prime\to t})
% \end{equation}



This term not only helps reduce error when a patch becomes occluded but also helps with patches no longer visible due to camera motion.\\

Owing to the image warping loss our Model currently assumes our surroundings are static as otherwise an object in motion cannot be correctly reprojected during our loss calculation. This however proves difficult in real world images where other cars, pedestrians and cyclists all move relative to us. This is amplified in sequences where the ego car is stationary for a preiod of time as image warping relies on pose changing. In Zhou et al.\cite{zhou2017} a predictive mask is used learn pixels containing objects which typically move compared to us. Monodepthv2\cite{monodepthv2} however implements auto-masking stationary pixels which works by applying a binary mask to image reconstruction loss which removes loss in pixels where the image has stayed the same between frames. This allows us to discount a whole image where the ego car is stationary, remove objects moving with similar velocity to ourselves (which causes infinite depth otherwise) or low texture regions which don't provide much information for an image similarity loss. This mask $\mu$ is thus calculated as

which ignores the loss of pixels when the reprojection error of the original unwarped source image $I_{t\prime}$ is lower than the warped image $I_{t\prime\to t}$. $[ ]$ indicates the Iverson bracket.

Multi-scale estimation
Final training Loss
Additional Considerations


Network Part training Ablation on Eigen Test. Here 10 steps of Stochastic Gradient Descent are performed with learning rate 0.1 on images in the Eigen test set with weights being reset to those of Monodepth2 after each image


In supervised learning training requires knowledge of ground truth output values, in our self-supervised network we however do not. This means that creating datasets for such networks only requires us to record a sequence of frames from a moving camera. While large collections of data are available to train on these datasets are prone to oversampling driving situations present in the countries of their creation, for example vegetation, building design, traffic signs and road furniture can all vary vastly between and within countries. As our network is trained to understand the scale of objects it has observed during training predictions for out of distribution situations suffer greatly. However owing to the self-supervised nature of our training we can overcome these issues of dissimilarity to the training set by performing some learning on the inference device which allows our network to better understand it's surroundings and develop a deeper understanding of it's own locality.\\


==> tables/sequential-results.tex <==
\begin{table}[t!]
     \caption{Comparison of resetting techniques. In the first Group of experiments weights are not reset to those of Monodepth 2 after each image is processed. The second grouping resets to Monodepths weights with the last grouping only returning once a new sequence in the Eigen Evaluation set is being evaluated}
  \centering
  \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
  \hline
  Strategy  & \cellcolor{col1}Abs Rel & \cellcolor{col1}Sq Rel & \cellcolor{col1}RMSE  & \cellcolor{col1}RMSE log & \cellcolor{col2}$\delta < 1.25 $ & \cellcolor{col2}$\delta < 1.25^{2}$ & \cellcolor{col2}$\delta < 1.25^{3}$ \\
  
  \hline

Monodepth 2 & 0.115 & 0.905 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981  \\
LSTM paper & 0.111 & 0.821 & 4.65 & 0.187 & 0.883 & 0.961 & 0.982  \\
\arrayrulecolor{grey}\hline

Instance-wise & 0.089 & 0.747 & 4.275 & 0.173 & 0.912 & 0.964 & 0.982  \\
Sequential    & 0.096 & 0.913 & 4.425 & 0.18 & 0.902 & 0.957 & 0.978  \\

% can add numbers for Stereo and M+S and different Sizes/Learning Rates


\arrayrulecolor{black}\hline

  \end{tabular}
  
 \label{tab:seq}
 \vspace{-10pt}
\end{table}
